Secure Computation to Hide Functions of Inputs

We consider a two-user secure computation problem in which Alice and Bob communicate interactively in order to compute some deterministic functions of the inputs. The privacy requirement is that each user should not learn any additional information about a function of the inputs other than what can be inferred from its own input and output. For the distribution-free setting, i.e., when the protocol must be correct and private for any joint input distribution, we completely characterize the set of all securely computable functions. When privacy is required only against Bob who computes a function based on a single transmission from Alice, we show that asymptotically secure computability is equivalent to perfectly secure computability. Separately, we consider an eavesdropper who has access to all the communication and should not learn any information about some function of the inputs (possibly different from the functions to be computed by the users) and show that interaction may be necessary for secure computation.

==> problem_statement.tex <==
\section{Problem Statement}

Alice and Bob have $X^n$ and $Y^n$, respectively, as their inputs, where $(X_i,Y_i)$, $i=1,\dots, n$, are independent and identically distributed (i.i.d.) with distribution $q_{XY}$.  Let $f(x,y),g(x,y)$ and $h(x,y)$ denote three deterministic functions of $x,y$. The users interactively communicate in $r$ rounds over a noiseless bidirectional link. They want to compute $Z_1^n$ and $Z_2^n$ so that, with high probability, they are equal to the functions $F^n$ and $G^n$, respectively, where $F_i=f(X_i,Y_i)$ and $G_i=g(X_i,Y_i)$ for $i=1\dots, n$. The secrecy requirement is that the average amount of information that the eavesdropper learns about $H^n$ $($with $H_i=h(X_i,Y_i)$$)$ from the communication vanishes asymptotically. Next, we formally state the problem.

\begin{defn}
A \emph{protocol} $\Pi_n$ with $r$ interactive rounds of communication consists of 
\begin{itemize}
\item a set of $r$ randomized encoders with p.m.f.'s $p^{\emph{E}_1}(m_i|x^n,m_{[1:i-1]})$ for odd numbers $i\in[1:r]$ 
and $p^{\emph{E}_2}(m_i|y^n,w,m_{[1:i-1]})$ for even numbers $i\in[1:r]$, where $M_i$ is the message transmitted in the $i^{\emph{th}}$ round,
\item two randomized decoders $p^{\emph{D}_1}(z_1^n|x^n,m_{[1:r]})$ and $p^{\emph{D}_2}(z_2^n|y^n,m_{[1:r]})$.
\end{itemize}
\end{defn}
Let $p^{\text{(induced)}}_{X^n,Y^n,M_{[1:r]},Z_1^n,Z_2^n}$ denote the induced distribution of the protocol $\Pi_n$.
\begin{align}
&p^{\text{(induced)}}(x^n,y^n,m_{[1:r]},z_1^n,z_2^n)=\frac{1}{2^{nR_0}}\prod_{i=1}^n q(x_i,y_i) \times\nonumber\\
&\left[\prod_{i:\text{odd}}p^{\text{E}_1}(m_i|x^n,m_{[1:i-1]})\prod_{j:\text{even}}p^{\text{E}_2}(m_j|y^n,m_{[1:j-1]})\right]\nonumber\\
&\times p^{\text{D}_1}(z_1^n|x^n,m_{[1:r]})p^{\text{D}_2}(z_2^n|y^n,m_{[1:r]})\label{eqn:induced}.
\end{align}

\begin{defn}
$(q_{XY},f,g,h)$ is \emph{asymptotically securely computable} in $r$ rounds if there exists a sequence of protocols $\Pi_n$ such that, for every $\epsilon>0$, there exists a large enough $n$ such that
\begin{align}
P(Z_1^n\neq F^n \ \emph{or}\  Z_2^n\neq G^n)&\leq \epsilon,\label{eqn:correctness}\\
I(M_{[1:r]};H^n)&\leq n\epsilon\label{eqn:security}.
\end{align}
\end{defn}
%\begin{remark}\label{remark:tyagi}
%Notice that the problem considered in this paper reduces to that of Tyagi et al. \cite{TyagiNG11} if $f=g=h$ and when the secrecy condition \eqref{eqn:security} is replaced by the following stronger requirement:
%\begin{align}
%I(M_{[1:r]};H^n)\leq \epsilon\label{eqn:stronger_security}.
%\end{align}
%\end{remark}
\begin{defn}
$(q_{XY},f,g,h)$ is \emph{perfectly securely computable} in $r$ rounds if there exists a protocol $\Pi_n$ with $n=1$ such that \eqref{eqn:correctness}-\eqref{eqn:security} are satisfied with $\epsilon=0$.
\end{defn}
\begin{defn}
An $(n,R_{12},R_{21})$ \emph{protocol} is a protocol $\Pi_n$ such that
\begin{align*}
R_{12}&=\frac{1}{n}\sum_{i:\emph{odd}}\log|\mathcal{M}_i|,\\
R_{21}&=\frac{1}{n}\sum_{i:\emph{even}}\log|\mathcal{M}_i|,
\end{align*}
where $\mathcal{M}_i$ is the alphabet of $M_i$, $i\in[1:r]$.
\end{defn}
For a given quadruple $(q_{XY},f,g,h)$, a rate pair $(R_{12},R_{21})$ is said to be achievable in $r$ rounds if there exists a sequence of $(n,R_{12},R_{21})$ protocols such that for every $\epsilon>0$, there exists a large enough $n$ satisfying \eqref{eqn:correctness}-\eqref{eqn:security}. The rate region $\mathcal{R}(r)$ is the closure of all the achievable rate pairs $(R_{12},R_{21})$ in $r$ rounds.


